Absynthe: Abstract Interpretation-Guided Synthesis

Synthesis tools have seen significant success in recent times. However, past approaches often require a complete and accurate embedding of the source language in the logic of the underlying solver, an approach difficult for industrial-grade languages. Other approaches couple the semantics of the source language with purpose-built synthesizers, necessarily tying the synthesis engine to a particular language model. In this paper, we propose Absynthe, an alternative approach based on user-defined abstract semantics that aims to be both lightweight and language agnostic, yet effective in guiding the search for programs. A synthesis goal in Absynthe is specified as an abstract specification in a lightweight user-defined abstract domain and concrete test cases. The synthesis engine is parameterized by the abstract semantics and independent of the source language. Absynthe validates candidate programs against test cases using the actual concrete language implementation to ensure correctness. We formalize the synthesis rules for Absynthe and describe how the key ideas are scaled-up in our implementation in Ruby. We evaluated Absynthe on SyGuS strings benchmark and found it competitive with other enumerative search solvers. Moreover, Absynthe's ability to combine abstract domains allows the user to move along a cost spectrum, i.e., expressive domains prune more programs but require more time. Finally, to verify Absynthe can act as a general purpose synthesis tool, we use Absynthe to synthesize Pandas data frame manipulating programs in Python using simple abstractions like types and column labels of a data frame. Absynthe reaches parity with AutoPandas, a deep learning based tool for the same benchmark suite. In summary, our results demonstrate Absynthe is a promising step forward towards a general-purpose approach to synthesis that may broaden the applicability of synthesis to more $\ldots$

==> extra.tex <==
\begin{comment}
\paragraph{Synthesizing programs over integers.}

\begin{figure}
\begin{center}
  $$
  \begin{array}{lccl}
  \emph{Values} \quad
  & \val
  & ::= & 0 \spmid 1 \spmid 2 \\
  \emph{Expressions} \quad
  & \expr
  & ::= & \val \spmid \var \spmid \expr + \expr \spmid \expr - \expr \\
  & & \spmid & \expr \times \expr \spmid \expr / \expr\\
  \emph{Programs} \quad
  & \program
  & ::= & \eprog{\meth}{\var}{\expr} \\
  \end{array}
  $$

  \caption{Syntax and types of \intlang{}.}
  \label{fig:intlang-syntax}
\end{center}
\end{figure}

Figure~\ref{fig:intlang-syntax} shows a tiny language \intlang
that has integers: 0, 1, 2, arithmetic operators of addition,
subtraction, multiplication, and division. Programs in \intlang take a
variable \var as argument and evaluate expression \expr. We will work
with a trivial example in this section to demonstrate how our synthesis
approach will work.

Suppose we want to synthesize a program that satisfies these
input/output pairs $\textsf{3} \mapsto \textsf{7}$, and $\textsf{4}
\mapsto \textsf{9}$. A simple way to
find the correct program will be start enumerating terms in the language
and then evaluate them with these input/output examples to test if an
enumerated program is correct. However, looking at these examples, we
can come up with a more abstract property that satisfies our examples:
$\top \rightarrow \odd$, i.e. we want a program that accepts any
number and produces an odd number. Do note that this property does not
encode all the information provided by the input/output examples, this
is an over-approximate specification, while the input-output examples
give concrete values.

We propose building simple program analyzers on top of our language,
enabling the synthesizer to accept such properties of the program that
can be automatically checked by the analyzer. Such a specification can
be used to efficiently guide the search for the correct solution.
For purposes of this example, we will define a parity analysis for our
language \intlang. Given a program \program in \intlang, the parity
analysis will compute if the produced number will be odd or even. To
begin, we define an abstract domain for parity $\mathbb{P} := \{\odd,
\even\}$. Values in \intlang can then be represented as $\bot$ (neither
odd nor even), \odd, \even, $\top$ (either odd or even).


\begin{figure}
\begin{center}
  \begin{align*}
    \bot  + \_    &:= \bot  \\
    \odd  + \even &:= \odd  \\
    \odd  + \odd  &:= \even \\
    \even + \even &:= \even \\
    \top  + \_    &:= \top  \\
  \end{align*}

  \caption{Rules for + operation over the parity domain.}
  \label{fig:parity-rules}
\end{center}
\end{figure}

It is then a matter of representing the language semantics over our
domain. Figure~\ref{fig:parity-rules} shows the semantics for
$\expr + \expr$ terms. Similar rules with left and right operands
flipped have been omitted, since addition is a commutative operation.
The $\_$ in the definitions can be substituted with any value. Similar
rules can be written for all other arithmetic operators $-, \times$, and
$/$. The key thing to note here, is that each of these abstraction, \odd
or \even, represent an infinite set of numbers. Thus reason over an
abstract domain, enables us to quickly work through the state space of
all possible programs. Semantics for $+$, $\times$, $/$ over parity
domain has been omitted for brevity.

Just like with \rbsyn, we start off with a hole $\ehole: \odd$, and initial
environment $\Gamma[\var \mapsto \top]$. In this setting, \absynthe asks
the question, what terms can yield \odd values? The semantics for
addition yields us two possible terms: $\odd + \even$ and
$\bot + \_$. The latter term simply means, if any non-integer value is
added to anything, we might get a non-integer value. While clearly all
values in our languages are integers, the mechanism to have $\bot$ rules
allows us to express semantics when some value cannot be lifted to the
abstract domain. Moving forward with the alternative, we can substitute
it with more holes to yield: $\ehole: \odd + \ehole: \even$. The choice
to substitute the holes here can give rise to multiple options, a few of
which are:

$$
\var + \var
\qquad
\var + 0
\qquad
\var + 1
\qquad
\ehole: \even + 1
\qquad
\ehole: \odd + 0
$$

All of these expressions can evaluate to an \odd number. On the other
hand, \absynthe{} could eliminate expressions like $\ehole: \even + 0$
and $\ehole: \odd + 1$ as these will always evaluate to \even values.

\absynthe will consider all expressions just like \rbsyn, eventually
trying $\ehole: \even + 1$. Similarly filling the \even hole here with
the rules for multiplication will give $(\ehole: \odd \times \ehole:
\even) + 1$, $(\ehole: \even \times \ehole: \even) + 1$, and $(\ehole:
\top \times \ehole: \even) + 1$. One of the possible substitution of the
holes in last template will be $(\var \times 2) + 1$, which is the
correct solution as it gives the correct result on input/output
examples. I only show the choices that lead to correct solution for
conciseness, but \absynthe{} will try all expressions.

An obvious question now would be why go through all the trouble just to
synthesize such a simple expression? To demonstrate the domains where
these approaches shine, I will take an example from the \sygus 2017 strings
benchmark suite~\cite{alur2017sygus}.
\end{comment}


---------------


% \begin{figure}
%   \centering
%   \begin{subfigure}{0.49\textwidth}
%   \begin{mathpar}
%   \inference{
%     \Gamma \vdash \expr_1 \Downarrow \strtype \\
%     \Gamma \vdash \expr_2 \Downarrow \inttype \qquad
%     \Gamma \vdash \expr_3 \Downarrow \inttype}
%     {\Gamma \vdash (\texttt{substr}\ \expr_1\ \expr_2\ \expr_3) \Downarrow
%     \strtype}[\rulename{T-Substr}]

%   \inference{
%       \Gamma \vdash \expr \Downarrow \strtype}
%      {\Gamma \vdash (\texttt{len}\ \expr)\Downarrow \inttype}[\rulename{T-Len}]

%   \inference{
%       \Gamma \vdash \expr_1 \Downarrow \inttype \qquad
%       \Gamma \vdash \expr_2 \Downarrow \inttype}
%      {\Gamma \vdash (-\ \expr_1\ \expr_2) \Downarrow \inttype}[\rulename{T-Sub}]

%   \inference{
%       \Gamma \vdash \expr_1 \Downarrow \strtype \qquad
%       \Gamma \vdash \expr_2 \Downarrow \strtype}
%      {\Gamma \vdash (\texttt{contains}\ \expr_1\ \expr_2) \Downarrow \booltype}[\rulename{T-Contains}]
%   \end{mathpar}
%   \caption{Selected rules using types as abstraction.}
%   \label{fig:absynthe-strlang-types}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.49\textwidth}
%     \begin{mathpar}
%     \inference{
%       \Gamma \vdash \expr_1 \Downarrow \strlenval_1
%       \qquad
%       \Gamma \vdash \expr_2 \Downarrow \strlenval_2 \\
%       \Gamma \vdash \expr_3 \Downarrow \strlenval_3
%       \qquad
%       \strlenval_3 \geq \strlenval_2
%       \qquad
%       \strlenval_1 \geq \strlenval_3}
%       {\Gamma \vdash (\texttt{substr}\ \expr_1\ \expr_2\ \expr_3) \Downarrow
%       \strlenval_3 - \strlenval_2}[\rulename{L-Substr}]

%     \inference{
%         \Gamma \vdash \expr \Downarrow \strlenval}
%        {\Gamma \vdash (\texttt{len}\ \expr) \Downarrow \bot}[\rulename{L-Len}]

%     \inference{
%         \Gamma \vdash \expr_1 \Downarrow \bot \qquad
%         \Gamma \vdash \expr_2 \Downarrow \bot}
%         {\Gamma \vdash (-\ \expr_1\ \expr_2) \Downarrow
%         \bot}[\rulename{L-Sub}]

%     \inference{
%         \Gamma \vdash \expr_1 \Downarrow \strlenval_1 \qquad
%         \Gamma \vdash \expr_2 \Downarrow \strlenval_2}
%        {\Gamma \vdash (\texttt{contains}\ \expr_1\ \expr_2) \Downarrow \bot}[\rulename{L-Contains}]
%     \end{mathpar}
%     \caption{Selected rules using string lengths as abstraction.}
%     \label{fig:strlang-strlen}
%   \end{subfigure}
%   \caption{\strlang semantics using types and string lengths domain.}
% \end{figure}

Figure~\ref{fig:absynthe-strlang-types} shows typing rules for \strlang.
Like \rbsyn, if we go from the conclusion to the premise of these rules
we will always synthesize type-correct programs. Similarly,
figure~\ref{fig:strlang-strlen} shows the semantics
when strings are lifted to their string lengths. Rules \rulename{L-Substr}
and \rulename{L-Sub} need some discussion. In \rulename{L-Substr} the
constraints with $\geq$ ensures that the index from which substring will
be extracted is within bounds of original string and the first index of
substring is less than the end index. For brevity, I have omitted rules
where $\strlenval_1$, $\strlenval_2$, and $\strlenval_3$ can evaluate to
$\bot$ or $\top$. In such cases the term $(\texttt{substr}\ \expr\
\expr)$ evaluates to $\bot$ and $\top$ respectively. \rulename{L-Sub}
might seem unsound, because the $-$ operation is on integers, whereas we
are operating on abstractions of strings, but when taken together with
the typing rules from figure~\ref{fig:absynthe-strlang-types}, the
string length abstraction will be used as integers in a sound fashion.
We can think of these two rule sets as an interpreter that computes
types and the length of output string. We will cast the synthesis
problem as a query to these interpreters: what expressions can evaluate
to the synthesis goal?
